Text-Augmented Open Knowledge Graph Completion via Pre-Trained Language Models

The mission of open knowledge graph (KG) completion is to draw new findings from known facts. Existing works that augment KG completion require either (1) factual triples to enlarge the graph reasoning space or (2) manually designed prompts to extract knowledge from a pre-trained language model (PLM), exhibiting limited performance and requiring expensive efforts from experts. To this end, we propose TAGREAL that automatically generates quality query prompts and retrieves support information from large text corpora to probe knowledge from PLM for KG completion. The results show that TAGREAL achieves state-of-the-art performance on two benchmark datasets. We find that TAGREAL has superb performance even with limited training data, outperforming existing embedding-based, graph-based, and PLM-based methods.

==> kge_repro_med.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[!h]
\small
\centering
\setlength{\tabcolsep}{3.9pt}
\resizebox{0.8\textwidth}{!}{\begin{tabular}{lllll}
\toprule
     & \multicolumn{2}{m}{\citeauthor{fu-etal-2019-collaborative}'s setting}     & \multicolumn{2}{m}{Our setting}            \\       
Model           & (edim, rdim, filter) & Ratio: (Hits@5, Hits@10)        & (edim, rdim, filter) & Ratio: (Hits@5, Hits@10)               \\    
\midrule
\midrule
TransE \cite{bordes2013translating}             & (100, 100, n/a)   & 20\%: (7.12, 11.17)   & (600, 600, n/a)   & 20\%: (19.70, 30.47)        \\
                                                && 40\%: (26.86, 38.08) && 40\%: (27.72, 41.99)         \\
                                                && 70\%: (31.32, 43.58) && 70\%: (34.62, 49.29)         \\
                                                && 100\%: (32.28, 45.52) && 100\%: (40.83, 53.62)          \\
\midrule  
DisMult \cite{yang2014embedding}             & (100, 100, n/a)   & 20\%: (14.66, 21.16)   & (600, 600, n/a)   & 20\%: (19.02, 28.35)        \\
                                                && 40\%: (26.90, 38.35) && 40\%: (28.28, 40.48)         \\
                                                && 70\%: (31.65, 44.98) && 70\%: (32.66, 47.01)         \\
                                                && 100\%: (32.80, 47.50) && 100\%: (39.53, 53.82)          \\
\midrule
ComplEx \cite{trouillon2016complex}             & (100, 100, n/a)   & 20\%: (18.18, 19.58)   & (600, 600, n/a)   & 20\%: (11.28, 17.17)        \\
                                                && 40\%: (23.77, 34.15) && 40\%: (24.64, 35.15)         \\
                                                && 70\%: (30.04, 43.60) && 70\%: (25.89, 38.19)         \\
                                                && 100\%: (31.84, 46.57) && 100\%: (34.54, 49.30)          \\
\midrule
ConvE \cite{dettmers2018convolutional}          & (200, 200, n/a)   & 20\%: (20.51, 30.11)   & (200, 200, n/a)   & 20\%: (20.45, 30.72)        \\
                                                && 40\%: (28.01, 42.04) && 40\%: (27.90, 42.49)         \\
                                                && 70\%: (31.01, 45.81) && 70\%: (30.67, 45.91)         \\
                                                && 100\%: (30.35, 45.35) && 100\%: (29.85, 45.68)          \\
                                                \cmidrule{4-5}
                                                &&& (600, 600, n/a) & 20\%: (20.26, 30.29) \\
                                                &&&& 40\%: (26.85, 41.57) \\
                                                &&&& 70\%: (26.97, 42.44) \\
                                                &&&& 100\%: (25.43, 41.58) \\
\midrule
TuckER \cite{balavzevic2019tucker}              & - & - & (100, 100, n/a)    & 20\%: (5.13, 8.06)        \\
                                                &&&&  40\%: (20.48, 31.20)         \\
                                                &&&&  70\%: (29.66, 42.89)          \\
                                                &&&& 100\%: (31.56, 44.72)         \\
                                                \cmidrule{4-5}
                                                &&& (256, 256, n/a) & 20\%: (19.94, 30.82) \\
                                                &&&& 40\%: (25.79, 41.00) \\
                                                &&&& 70\%: (26.48, 42.48)               \\
                                                &&&& 100\%: (30.22, 45.33) \\
                                                \cmidrule{4-5}
                                                &&& (600, 600, n/a) & 20\%: (18.84, 27.94) \\
                                                &&&& 40\%: (24.57, 37.79) \\
                                                &&&& 70\%: (25.50, 41.32)               \\
                                                &&&& 100\%: (24.41, 40.56) \\
                                                
\midrule
RotatE \cite{sun2018rotate}                     & (200, 100, n/a)    & 20\%: (4.03, 6.50)    & (600, 600, n/a)    & 20\%: (17.95, 27.55)        \\
                                                && 40\%: (8.65, 13.21)  &&  40\%: (27.35, 40.68)         \\
                                                && 70\%: (14.90, 21.67) && 70\%: (34.81, 48.81) \\
                                                && 100\%: (20.75, 27.82) && 100\%: (40.15, 53.82)         \\
\bottomrule
\end{tabular}}
\caption{\textbf{Performance evaluation of knowledge graph embedding (KGE) models on UMLS-PubMed dataset}}
\label{tb:5}
\end{table*}

==> perf_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[t]
\small
\centering
\setlength{\tabcolsep}{3.9pt}
\begin{tabular}{lccccccccc}
\toprule
Model      & \multicolumn{3}{m}{20\%}     & \multicolumn{3}{m}{50\%}     & \multicolumn{3}{m}{100\%}            \\       
           & Hits@5 & Hits@10 & MRR       & Hits@5 & Hits@10 & MRR       & Hits@5 & Hits@10 & MRR               \\    
\midrule
\midrule
TransE \cite{bordes2013translating}             & 15.12    & 18.83    & 12.57    & 19.38    & 23.20    & 13.36    & 38.53    & 43.38    & 29.90    \\
DisMult \cite{yang2014embedding}                & 1.42     & 2.55     & 1.05     & 15.23    & 19.05    & 12.36    & 32.11    & 35.88    & 24.95    \\
ComplEx \cite{trouillon2016complex}             & 4.22     & 5.97     & 3.44     & 19.10    & 23.08    & 12.99    & 32.91    & 34.62    & 24.67    \\
ConvE \cite{dettmers2018convolutional}          & 20.60    & 26.90    & 11.96    & 24.39    & 30.59    & 18.51    & 33.02    & 39.78    & 24.45    \\
TuckER \cite{balavzevic2019tucker}              & 21.35    & 24.80    & 18.51    & 31.25    & 33.06    & 27.52    & 46.53    & 48.92    & 43.06    \\
RotatE \cite{sun2018rotate}                     & 9.25     & 11.83    & 8.04     & 25.96    & 31.63    & 23.34    & 58.32    & 60.66    & 51.85    \\
\midrule
RC-Net \cite{xu2014rc}                          & 13.48    & 15.37    & 13.26    & 14.87    & 16.54    & 14.63    & 14.69    & 16.34    & 14.41    \\
TransE+Line \cite{fu-etal-2019-collaborative}   & 12.17    & 15.16    & 4.88     & 21.70    & 25.75    & 8.81     & 26.76    & 31.65    & 10.97    \\
JointNRE \cite{han2018neural}                   & 16.93    & 20.74    & 11.39    & 26.96    & 31.54    & 21.24    & 42.02    & 47.33    & 32.68    \\
\midrule
MINERVA \cite{das2017go}                        & 11.64    & 14.16    & 8.93     & 25.16    & 31.54    & 22.24    & 43.80    & 44.70    & 34.62    \\
CPL \cite{fu-etal-2019-collaborative}           & 15.19    & 18.00    & 10.87    & 26.81    & 31.70    & 23.80    & 43.25    & 49.50    & 33.52    \\
\midrule
PKGC \cite{lv2022pre}                           &          &          &          &          &          &          &          &          &          \\
TagReal w/ (Man + Supp)                         &          &          &          &          &          &          &          &          &          \\
TagReal w/ (Mine + Supp)                        &          &          &          &          &          &          &          &          &          \\
TagReal w/ (Optim + Supp)                       &          &          &          &          &          &          &          &          &          \\ 
\bottomrule
\end{tabular}
\caption{\textbf{Performance comparison on KG reasoning on FB60K-NYT10 dataset}. The highest score for each metric in different sub-train-sets is highlighted in \textbf{bold.}}
\label{tb:1}
\end{table*}
